Local time steps for a finite volume scheme

We present a strategy for solving time-dependent problems on grids with local refinements in time using different time steps in different regions of space. We discuss and analyze two conservative approximations based on finite volume with piecewise constant projections and domain decomposition techniques. Next we present an iterative method for solving the composite-grid system that reduces to solution of standard problems with standard time stepping on the coarse and fine grids. At every step of the algorithm, conservativity is ensured. Finally, numerical results illustrate the accuracy of the proposed methods.

==> maillage_DF.tex <==
\begin{picture}(160,150)

% lignes horizontales
\matrixput(0,20)(1,0){1}(0,10){11}{\line(1,0){80}}
\matrixput(80,20)(1,0){1}(0,50){3}{\line(1,0){80}}

% lignes verticales
\matrixput(0,20)(10,0){7}(0,10){1}{\line(0,1){100}}
\matrixput(80,20)(20,0){5}(0,50){1}{\line(0,1){100}}

% axes
\put(160,20){\vector(1,0){10}}
\put(172,15){\makebox(10,10){x}}
\put(0,120){\vector(0,1){10}}
\put(-5,132){\makebox(10,10){t}}

% temps discrets
\put(-12,65){\makebox(10,10){$t_n$}}
\put(-12,75){\makebox(10,10){$t_{n,1}$}}
\put(-12,85){\makebox(10,10){$t_{n,2}$}}
\put(-12,95){\makebox(10,10){$t_{n,3}$}}
\put(-12,105){\makebox(10,10){$t_{n,4}$}}
\put(-12,115){\makebox(10,10){$t_{n+1}$}}

% position des inconnues
\matrixput(5,20)(10,0){6}(0,10){11}{\circle{3}}
\matrixput(70,20)(10,0){1}(0,10){11}{\circle{3}}
\matrixput(90,20)(20,0){4}(0,50){3}{\circle{3}}

\end{picture}


==> maillage_VF.tex <==
\begin{picture}(160,150)

% lignes horizontales
\matrixput(0,20)(1,0){1}(0,10){11}{\line(1,0){80}}
\matrixput(80,20)(1,0){1}(0,50){3}{\line(1,0){80}}

% lignes verticales
\matrixput(0,20)(10,0){7}(0,10){1}{\line(0,1){100}}
\matrixput(80,20)(20,0){5}(0,50){1}{\line(0,1){100}}

% axes
\put(160,20){\vector(1,0){10}}
\put(172,15){\makebox(10,10){x}}
\put(0,120){\vector(0,1){10}}
\put(-5,132){\makebox(10,10){t}}

% temps discrets
\put(-12,70){\makebox(10,10){$t_{n,1}$}}
\put(-12,80){\makebox(10,10){$t_{n,2}$}}
\put(-12,90){\makebox(10,10){$t_{n,3}$}}
\put(-12,100){\makebox(10,10){$t_{n,4}$}}
\put(-12,110){\makebox(10,10){$t_{n,5}$}}
\put(165,65){\makebox(10,10){$t_{n-\frac{1}{2}}$}}
\put(165,115){\makebox(10,10){$t_{n+\frac{1}{2}}$}}
\put(165,40){\makebox(10,10){$t_{n-1}$}}
\put(163,90){\makebox(10,10){$t_n$}}

% pas de temps
\put(-3,45){\vector(0,1){5}}
\put(-3,45){\vector(0,-1){5}}
\put(-15,40){\makebox(10,10){$\dt_1$}}
\put(185,45){\vector(0,1){25}}
\put(185,45){\vector(0,-1){25}}
\put(190,40){\makebox(10,10){$\dt_2$}}

% position des inconnues
\matrixput(5,25)(10,0){6}(0,10){10}{\circle{3}}
\matrixput(70,25)(10,0){1}(0,10){10}{\circle{3}}
\matrixput(90,45)(20,0){4}(0,50){2}{\circle{3}}

% inconnues d'interface
\matrixput(75,20)(1,0){1}(0,10){10}{\makebox(10,10){\small $\varoslash$}}
\matrixput(75,40)(1,0){1}(0,50){2}{\makebox(10,10){\small $\varobslash$}}

\end{picture}


==> maillage_VF_rec.tex <==
\begin{picture}(160,150)

% lignes horizontales
\matrixput(0,20)(1,0){1}(0,10){11}{\line(1,0){80}}
\matrixput(80,20)(1,0){1}(0,50){3}{\line(1,0){80}}

% lignes verticales
\matrixput(0,20)(10,0){7}(0,10){1}{\line(0,1){100}}
\matrixput(80,20)(20,0){5}(0,50){1}{\line(0,1){100}}

% axes
\put(160,20){\vector(1,0){10}}
\put(172,15){\makebox(10,10){x}}
\put(0,120){\vector(0,1){10}}
\put(-5,132){\makebox(10,10){t}}

% temps discrets
\put(-12,70){\makebox(10,10){$t_{n,1}$}}
\put(-12,80){\makebox(10,10){$t_{n,2}$}}
\put(-12,90){\makebox(10,10){$t_{n,3}$}}
\put(-12,100){\makebox(10,10){$t_{n,4}$}}
\put(-12,110){\makebox(10,10){$t_{n,5}$}}
\put(165,65){\makebox(10,10){$t_{n-\frac{1}{2}}$}}
\put(165,115){\makebox(10,10){$t_{n+\frac{1}{2}}$}}
\put(165,40){\makebox(10,10){$t_{n-1}$}}
\put(163,90){\makebox(10,10){$t_n$}}

% pas de temps
\put(-3,45){\vector(0,1){5}}
\put(-3,45){\vector(0,-1){5}}
\put(-15,40){\makebox(10,10){$\dt_1$}}
\put(185,45){\vector(0,1){25}}
\put(185,45){\vector(0,-1){25}}
\put(190,40){\makebox(10,10){$\dt_2$}}

% position des inconnues
\matrixput(5,25)(10,0){6}(0,10){10}{\circle{3}}
\matrixput(70,25)(10,0){1}(0,10){10}{\circle{3}}
\matrixput(90,45)(20,0){4}(0,50){2}{\circle{3}}

% inconnues d'interface
\matrixput(85,20)(1,0){1}(0,10){10}{\makebox(10,10){\small $\varoslash$}}
\matrixput(65,40)(1,0){1}(0,50){2}{\makebox(10,10){\small $\varobslash$}}

% definition d1 et d2
\put(70,15){\vector(1,0){10}}
\put(70,15){\vector(-1,0){10}}
\put(65,5){\makebox(10,10){$2d_\eps^1$}}
\put(90,15){\vector(1,0){10}}
\put(90,15){\vector(-1,0){10}}
\put(85,5){\makebox(10,10){$2d_\eps^2$}}

\end{picture}


==> maillage_hm.tex <==
\begin{picture}(160,30)

% la discretisation
\put(0,20){\line(1,0){160}}
\matrixput(0,17.5)(10,0){7}(0,10){1}{\line(0,1){5}}
\matrixput(80,17.5)(20,0){5}(0,10){1}{\line(0,1){5}}

% definition des zones puits et reservoir
\put(40,10){\vector(1,0){40}}
\put(40,10){\vector(-1,0){40}}
\put(35,0){\makebox(10,10){(P)}}
\put(120,10){\vector(1,0){40}}
\put(120,10){\vector(-1,0){40}}
\put(115,0){\makebox(10,10){(R)}}

\end{picture}

